Faster Counting and Sampling Algorithms using Colorful Decision Oracle

In this work, we consider $d$-{\sc Hyperedge Estimation} and $d$-{\sc Hyperedge Sample} problem in a hypergraph $\mathcal{H}(U(\mathcal{H}),\mathcal{F}(\mathcal{H}))$ in the query complexity framework, where $U(\mathcal{H})$ denotes the set of vertices and $\mathcal{F}(\mathcal{H})$ denotes the set of hyperedges. The oracle access to the hypergraph is called {\sc Colorful Independence Oracle} ({\sc CID}), which takes $d$ (non-empty) pairwise disjoint subsets of vertices $A_1,\ldots,A_d \subseteq U(\mathcal{H})$ as input, and answers whether there exists a hyperedge in $\mathcal{H}$ having (exactly) one vertex in each $A_i, i \in \{1,2,\ldots,d\}$. The problem of $d$-{\sc Hyperedge Estimation} and $d$-{\sc Hyperedge Sample} with {\sc CID} oracle access is important in its own right as a combinatorial problem. Also, Dell {\it{et al.}}~[SODA '20] established that {\em decision} vs {\em counting} complexities of a number of combinatorial optimization problems can be abstracted out as $d$-{\sc Hyperedge Estimation} problems with a {\sc CID} oracle access. The main technical contribution of the paper is an algorithm that estimates $m= \lvert {\mathcal{F}(\mathcal{H})}\rvert$ with $\widehat{m}$ such that { $$ \frac{1}{C_{d}\log^{d-1} n} \;\leq\; \frac{\widehat{m}}{m} \;\leq\; C_{d} \log ^{d-1} n . $$ by using at most $C_{d}\log ^{d+2} n$ many {\sc CID} queries, where $n$ denotes the number of vertices in the hypergraph $\mathcal{H}$ and $C_{d}$ is a constant that depends only on $d$}. Our result coupled with the framework of Dell {\it{et al.}}~[SODA '21] implies improved bounds for a number of fundamental problems.

==> algo.tex <==
\section{Algorithm} \label{sec:algo}

\noindent In this Section we describe our algorithm for $(1 \pm \eps)$ multiplicative approximation of the number of hyperedges $m_o(\cH)$ in a hypergraph $\cH$. As mentioned earlier, when $\eps \leq \lbeps$, then we compute the exact value of $m_o(\cH)$ by querying $m_o(\{a_1\},\ldots,\{a_d\})$ for all distinct $a_1,\ldots,a_d\in U(\cH)$, and this requires only polylogarithmic number of queries. We do the following when $\eps > \lbeps$. We build a data structure $\cal D$ that maintains the following two quantities at any point of time.


\begin{itemize}
	\item[(i)] An accumulator $\Psi$ for the number of hyperedges. We initialize $\Psi=0$.
	\item[(ii)] A set of tuples $(A_{11},\ldots,A_{1d},w_1),\ldots,$ $(A_{\zeta 1},\ldots,A_{\zeta d},w_{\zeta})$ for some $\zeta>0$, where tuple $(A_{i1},\ldots,A_{id})$ corresponds to the $d$-partite subgraph $\cH(A_{i1},\ldots,A_{id})$ and $w_i$ is the weight associated to $\cH(A_{i1},\ldots,A_{id})$. 
\end{itemize}
The data structure is initialized with $\Psi=0$, and only one tuple $(U^{[d]},1)$. The Algorithm performs the following steps.
\begin{itemize}
	\item[(1)] When there are no tuples left in the data structure $\cal D$, the Algorithm outputs $\Psi$ as the estimate. 

	\item[(2)]{\bf (Exact Counting)} Fix a threshold $\tau $ as $\frac{k^2\cdot 4^{2d}\theta^{2d} \cdot 16d^2 \cdot d! \log ^{d+2} n}{\eps^2}$, where $k=4$~\footnote{We take $k=4$ for ease of calculations. The argument works for any $k$}. For each tuple $(A_1,\ldots,A_d,w)$ in $\cal D$, decide whether $m_o(\dsubset) \leq \tau$ using Lemma~\ref{lem:exact}. If $m_o(\dsubset) \leq \tau$, we add the weighted number of ordered hyperedges $w \cdot m_o(\dsubset)$ to $\Psi$ and remove $(A_1,\ldots,A_d,w)$ from $\cal D$. If there are no tuples left in $\cal D$, then go to Step $1$. Otherwise, if the number of tuples is at most $\cN=\kappa_d \cdot \frac{\log ^{4d} n}{\eps^2}$, then go to Step $3$, else go to Step $4$. Note that $\kappa_d$ is a constant to be fixed later. By Lemma~\ref{lem:exact}, the query complexity of Step $2$ is $\cO_d(\tau \log n)=\cO_d\left( \frac{\log^{d+3}n}{\eps^2}\right)$ per tuple.

	\item[(3)] {\bf (Sparsification)} For any tuple $(A_1^{[a_1]},\ldots,A_s^{[a_s]},w)$ here we have $m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})>\tau$. Note that $A_i$ and $A_j$ are pairwise disjoint subsets for each $1\leq i <j \leq s$. We take $h_d:[k]^{d}\rightarrow \{0,1\}$ to be a hash function such that $\pr\left(h_d({\bf a}=1)\right)=1/k$ independently for each tuple ${\bf a} \in [k]^d$. The vertices in $A=\bigcup\limits_{i=1}^s A_i$ are \colored with $[k]=[4]$, and let $\chi(i,j)=\{v \in A_i~:~v~\mbox{is \colored with color $j$}\},$, where $i \in [s]$ and $j \in [k]$. We add each tuple $\left(\chi({1,c_1}),\ldots,\chi({1,c_{a_1}}),\ldots, \chi({s,c_{d-a_s+1}}),\ldots,\chi({s,c_{d}}),4w\right)$ to $\cal D$ for which $h_d(c_1,\ldots,c_d)=1$. We remove the tuple $(A_1^{[a_1]},\ldots,A_s^{[a_s]},w)$ from $\cal D$. After processing all the tuples, we go to Step $2$. Note that no query is required in Step $3$. The constant $4$ is obtained by putting $k=4$ in Lemma~\ref{lem:sparse2}.

	\item[(4)] ({\bf Coarse Estimation}) Let $r>\cN=\frac{\kappa_d\log^{4d} n}{\eps^2}$. Let $\{(A_{i1},\ldots,A_{id},w_i):i \in [r]\}$ be the set of tuples stored in $\cal D$. For each tuple $(A_{i1},\ldots,A_{id},w_i)$ in $\cal D$, we find an estimate $\hat{E_i}$ such that $\frac{m_o(A_1,\ldots,A_d)}{8\cdot 2^{d}d^{d-1} \log^{d-1} n} \leq \hat{E_i} \leq 20 \cdot 2^{d}d^{d-1} \log^{d-1} n \cdot m_o(A_1,\ldots,A_d)$. Lemma~\ref{lem:coarse_main} proves that this can be done with $\Oh_d(\log^{d+1} n)$ \gtwopis queries per tuple. We know that the number of tuples in $\cal D$ is more than $\cN=\kappa_d \frac{\log ^{4d} n}{\eps^2}$. We take a sample from the set of tuples such that the sample maintains the required estimate \emph{approximately} using Lemma~\ref{lem:importance-app}. This lemma follows from a lemma by Beame \etal~\cite{BeameHRRS18}. The original statement of the lemma by Beame et al.\ is given in Lemma~\ref{lem:importance1} in Appendix~\ref{sec:prelim}.

\begin{lem} \label{lem:importance-app} Let $\{(A_{i1},\ldots,A_{id},w_i):i \in [r]\}$ be the set of tuples in the data structure $\cal D$ and $e_i$ be the coarse estimation for $m_o(A_{i1},\ldots,A_{id},w_i)$ such that 
	\begin{itemize}
		\item[(i)] $w_i,e_i \geq 1~ \forall i \in [r]$
		\item[(ii)] $\frac{e_i}{\alpha} \leq m_o(A_{i1},\ldots,A_{id}) \leq e_i \cdot \alpha$ for some $\alpha >0$ and $\forall ~i \in [r]$
		\item[(iii)] $\sum_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})} \leq M$
	\end{itemize}
There exists an algorithm that finds a set $\{(A'_{i1},\ldots,A'_{id},w'_i):i \in [r']\}$ of tuples such that the above three conditions hold and $\size{\sum\limits_{i=1}^{r'} {w'_i\cdot m_o(A'_{i1},\ldots,A'_{id})}-\sum\limits_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})}} \leq \lambda S$ with probability $1-\delta$ where $S=\sum_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})}$ and $\lambda, \delta >0$. Also, $r'=\cO\left(\lambda^{-2} \alpha^4 \log M \left(\log \log M + \log \frac{1}{\delta}\right)\right)$. \end{lem} 

We use the algorithm for Lemma~\ref{lem:importance-app} with $\lambda =\frac{\eps}{4d \log n}$, $\alpha =  20 \cdot 2^{d}d^{d-1} \log^{d-1} n$ and $\delta = \frac{1}{n^{6d}}$ to find a new set  $\{(A'_{i1},\ldots,A'_{id},w'_i):i \in [r']\}$ of tuples satisfying the following: $\size{S-\sum_{i=1}^{r'} w'_i m_o(A'_{i1},\ldots,A'_{id})} \leq  \lambda S$ with probability $1-\frac{1}{n^{6d}}$, where $S=\sum_{i=1}^r w_i\cdot m_o(A_{i1},\ldots,A_{id})$. Here, $r'\leq \kappa_d \cdot \frac{\log ^{4d} n}{\eps^2}$. This $\kappa_d$ is same as the one mentioned in Step $2$. We remove the set of $r$ tuples$,r > \cN,$ from $\cal D$ and add the set of $r'$ tuples, where $r'\leq \kappa_d\cdot \frac{\log^ {4d} n}{\eps^2}=\cN$. As no query is required to execute the algorithm of Lemma~\ref{lem:importance-app}, the number of \gtwopis queries in this step in each iteration, is $\Oh_d(\log ^{d+1} n)$ per tuple. 

\end{itemize}


==> correct.tex <==
\section{Proof of Correctness} \label{sec:correct}
\noindent
We start with the following observation for the proof of correctness.
\begin{obs} \label{obs:num_tuples} There are at most $4^d\cdot \cN =4^d \kappa_d \cdot \frac{\log ^{4d} n}{\eps^2}$ tuples in the data structure $\cal D$ during the execution of the algorithm. \end{obs}

\begin{proof} The number of tuples in $\cal D$ can increase by a factor of $4^d$ in the sparsification step. Note that we apply the spasification step only when there are at most $\cN=\kappa_2 \cdot \frac{\log ^{4d} n}{\eps^2}$ many tuples in $\cal D$. Hence, the number of tuples in $\cal D$ is at most $4^d \cdot \cN$. \end{proof}

Now we prove Lemma~\ref{lem:prob1}. We restate the lemma for easy reference.
\begin{lem}[Lemma~\ref{lem:prob1} restated] \label{lem:prob} If $\eps \geq \lbeps$, our algorithm produces a $(1\pm \eps)$-approximation to $m_o(\cH)$ with probability at least $1-\frac{1}{n^{4d}}$ and makes $\Oh\left( \frac{\log ^{5d+4} n}{\eps^4}\right)$ queries, where each query is either a \gonepis query or a \gtwopis query. \end{lem}

To prove the above lemma, we need the following definition~\ref{defi:est} along with Observations~\ref{lem:iter1} and~\ref{lem:iter2}.

\begin{defi} \label{defi:est} Let $\mbox{{\sc Tuple}}_i$ be the set of tuples in $\cal D$ at the end of the $i$-th iteration. We {partition them into two parts --- a set of tuples $\tuple_i^{\leq \tau}$ and $\tuple_i^{>\tau}$ contributing less than and more than $\tau$ ordered hyperedges, respectively.}  Formally, $\tuple_i^{\leq \tau}=\{(A_1,\ldots,A_d,w):m_o(\dsubset) \leq \tau\}$ and $\tuple_i^{>\tau}=\tuple_{i} \setminus \tuple_i^{\leq \tau}$. Let $\Psi_i$ denote the value of $\Psi$ after the $i$-th iteration where $i \in \N$. The estimate for $m_o(\cH)=m_o(U^{[d]})$ after the $i$-th iteration is given as $\est_{i}=\Psi_i + \sum\limits_{(A_1,\ldots,A_d,w) \in \tuple_i} w \cdot m_o(\dsubset)$. The number of active hyperedges after the $i$-th iteration is given as $\act_{i}=\sum\limits_{(A_1,\ldots,A_d,w) \in \tuple_i} m_o(\dsubset)$. \end{defi}

Note that if there are some tuples left in $\cal D$ at the end of the $i$-th iteration, we do not know the value of $\est_i$ and $\act_i$. However, we know $\Psi_i$. Observe that $\Psi_{0}=0$ and $\est_{0}=\act_{0}=m_o(\cH)$.

\begin{obs} \label{lem:iter1} Let there be only one tuple in $\cal D$ after the $i$-th iteration for any non-negative integer $i$. Then, $\est_{{i+1}}$ is a $(1+\lambda)$-approximation to $\est_i$ {with probability at least $1-\frac{1}{n^{5d}}$}, where $\lambda=\frac{\eps}{4d \log n}$. \end{obs}

\begin{proof} From Definition~\ref{defi:est},
\begin{eqnarray*}
	\est_{i} &=& \Psi_i + \sum\limits_{(A_1,\ldots,A_d,w) \in \tuple_i} w\cdot m_o(\dsubset) \\
		 &=& \Psi_i + \sum\limits_{(A_1,\ldots,A_d,w) \in \tuple_i^{\leq \tau}} w\cdot m_o(\dsubset) + \sum\limits_{(A_1,\ldots,A_d,w) \in \tuple_i^{>\tau}} w\cdot m_o(\dsubset) 
\end{eqnarray*}

In Step $2$ of the algorithm, for each tuple $(\dsubset,w) \in \tuple_i^{\leq \tau}$, we determine the exact value of $m_o(\dsubset)$, add $w \cdot m_o(\dsubset)$ to the current value of $\Psi$ and remove the tuple from $\cal D$. Observe that
\begin{equation}
	\Psi_{i+1} -\Psi_i = \sum\limits_{(\dsubset,w)\in \tuple_i^{\leq \tau}}w\cdot m_o(\dsubset) \label{eqn:2}
\end{equation}

If $\tuple_i^{>\tau}$ is empty, we go to Step $1$ to report the output. Observe that in that case $\est_{i+1}=\est_i$, and we are done. If $\tuple_i^{>\tau}$ is non-empty, then we go to either Step $3$ or Step $4$ depending on whether the number of tuples in $\cal D$ is at most $\cN$ or more than $\cN$, respectively, where $\cN=\kappa_d\frac{\log ^{4d}n}{\eps^2}$.

	{\bf Case 1 (Go to Step $3$):} Note that for each tuple $(\dsubset,w)$ in $\cal D$, we have $\tuple_{i}^{\geq \tau}$. We apply the sparsification step (Step $3$) for each tuple. For each tuple $(\dsubset,w)$, we add a set of tuples $\cZ$ {(each tuple in $\cZ$ is of the form $(B_1,\ldots,B_d,4w)$)} by removing $(\dsubset,w)$ from $\cal D$. By Lemma~\ref{lem:sparse}, we have the following with probability $1-\frac{1}{n^{4\theta -2d}}$.
	$$\size{k\sum\limits_{(B_1,\ldots,B_d,4w) \in \cZ}m_o(B_1,\ldots,B_d) - m_o(\dsubset)} \leq k 2^{2d}\theta^d   \sqrt{ d! m_o(\dsubset) \log^d n}.$$ 
{Note that this is the same $k$ as that mentioned in Step 2 of our algorithm (see Section~\ref{sec:algo}). Moreover, $k=4$.}	
	%\complain{{(\bf $k$ on RHS was missing earlier} Gopi, I do not understand this comment.) But what is $k$ and where is it mentioned? Possibly, in earlier Section?}

	Now using $m_o(\dsubset) \geq \tau=\frac{k^2\cdot 4^{2d}\theta^{2d} \cdot 16d^2 \cdot d! \log ^{d+2} n}{\eps^2}~\mbox{and}~k=4$ and taking $\theta=2d$, we have Equation \ref{eqn:3} {holding} with probability $1-\frac{1}{n^{6d}}$.

\begin{equation}
	\size{\sum\limits_{(B_1,\ldots,B_d,4w) \in \cZ}4w \cdot m_o(B_1,\ldots,B_d) - w\cdot m_o(\dsubset)} \leq  \frac{\eps}{4d \log n}   \cdot w \cdot m_o(\dsubset) \label{eqn:3}
\end{equation}

	Since we are in Step $3$, there are at most $\cN=\kappa_d \frac{\log ^{4d} n}{\eps^2}$ many tuples in $\tuple_i^{>\tau}$. As $\eps > \left(\frac{\log^{5d+5}}{n^d}\right)^{1/4}$, the probability that Equation \ref{eqn:3} holds for each tuple in $\tuple_i^{>\tau}$ is at least $1-\frac{1}{n^{5d}}$.

By Definition~\ref{defi:est},
\begin{eqnarray*}
	\est_{i+1} &=& \Psi_{i+1} + \sum\limits_{(B_1,\ldots,B_d,w') \in \tuple_{i+1}} w' \cdot m_o(B_1,\ldots,B_d) 
\end{eqnarray*}

	Using Equations \ref{eqn:2} and \ref{eqn:3}, we can show that $\est_{i+1}$ is a $(1+\lambda)$-approximation to $\est_i$, where $\lambda=\frac{\eps}{4d \log n}$, and the probability of success is $1-\frac{1}{n^{5d}}$.

	{\bf Case $2$ (Go to Step $4$):} Here, we apply coarse estimation algorithm for each tuple $(\dsubset,w)$ present in $\cal D$ to find $\hat{E}$ such that $\frac{m_o(\dsubset)}{\alpha} \leq \hat{E} \leq \alpha \cdot  m_o(\dsubset)$ as described in Step-4. By Lemma~\ref{lem:coarse_main}, the probability of success of finding the required coarse estimation for a particular tuple, is at least $1-\frac{1}{n^{8d}}.$ By Observation~\ref{obs:num_tuples}, we have at most $4^d \cN =\frac{\kappa_d 4^d \log ^{4d} n}{\eps^2}$ many tuples at any instance of the algorithm. Hence, as $\eps > \left( \frac{\log ^{5d+5} n}{n^d}\right)^{1/4}$, the probability that we have the desired coarse estimation for all tuples present in $\cal D$, is at least $1-\frac{1}{n^{6d}}$.
 We have $r > \cN=\kappa_d \frac{\log ^{4d} n}{\eps^2}$ many tuples in $\cal D$. Under the conditional space that we have the desired coarse estimation for all tuples present in $\cal D$, we apply the algorithm {\sc Alg} corresponding to Lemma~\ref{lem:importance-app}. In doing so, we get $r' \leq \cN$ many tuples, as described in the Step-4, with probability $1-\frac{1}{n^{6d}}$. Observe that $\tuple_{i+1}$ is the set of $r'$ tuples returned by {\sc Alg} satisfying
 \begin{equation}\label{eqn:4}
 \size{ \sum\limits_{(B_1,\ldots,B_d,w')} w' \cdot m_o(B_1,\ldots,B_d) - S} 
  \leq \lambda S,
 \end{equation}
where $\lambda = \frac{\eps}{4d \log n}$ and $\sum\limits_{(\dsubset,w) \in \tuple_i^{>\tau}} w \cdot m_o(\dsubset)$. Now, by Definition~\ref{defi:est},
  \begin{eqnarray*}
  \est_{i+1} &=& \Psi_{i+1} + \sum\limits_{(B_1,\ldots,B_d,w') \in \tuple_{i+1}} w' \cdot m_o(B_1,\ldots,B_d) 
  \end{eqnarray*}
{Using Equations~\ref{eqn:2} and~\ref{eqn:4}}, we can show that $\est_{i+1}$ is a $(1+\lambda)$-approximation to $\est_i$ and the probability of success  is $1-\left(\frac{1}{n^{6d}}+\frac{1}{n^{6d}}\right)\geq 1-\frac{1}{n^{6d-1}}$.
\end{proof}


\begin{obs} \label{lem:iter2} Let there be at least one tuple $(A_1,\ldots,A_d,w)$ in the data structure $\cal D$ after the $i$-th iteration such that $m_o(\dsubset) > \tau$ for any integer $i>0$. Then, $\act_{{i+2}} \leq \frac{\act_{i}}{2}$ with probability at least $1-\frac{2}{n^{5d}}$. \end{obs}

\begin{proof}%[Proof of Observation~\ref{lem:iter2}]
As there exists one tuple in $\tuple_i^{>\tau}$, our algorithm will not terminate in Step-2. It will determine the exact values of
$m_o(\dsubset)$ for each $(\dsubset,w)\in \tuple_i^{\leq \tau}$, and then will go to either Step-2 or Step-3 depending on the cardinality of $\tuple_i^{\leq \tau}$. By adapting the same approach as that in the proof of Observation~\ref{lem:iter1}, we can show that
\begin{itemize}
\item[(i)] in the $(i+1)$-th iteration, if our algorithm goes to Step-3, then $\act_{i+1} \leq \frac{\act_{i}}{2}$ with probability $1-\frac{1}{n^{5d}}$; and
\item[(ii)] in the $(i+1)$-th iteration, if our algorithm goes to Step-4, then $\act_{i+1} \leq {\act_{i}}$ with probability $1-\frac{1}{n^{6d-1}}$.
\end{itemize}
From the description of the algorithm, it is clear that we apply sparsification either in iteration $(i+1)$ or $(i+2)$. That is, either we do sparsification in both the iterations, or we do sparsification in one iteration and coarse estimation in the other iteration, or we do sparsification in $(i+1)$-th iteration and termination of the algorithm after executing Step-2 in the $(i+2)$-th iteration. Observe that in the last case, that is, if we terminate in the $(i+2)$-th iteration, then $\act_{i+2}=0 \leq \frac{\act_{i}}{2}$. In the other two cases, by (i) and (ii), we have $\act_{i+2}\leq \frac{\act_i}{2}$ with probability at least $1-\frac{2}{n^{5d}}$.
\end{proof}


Now, we are ready to prove Lemma~\ref{lem:prob}.

\begin{proof}[Proof of Lemma~\ref{lem:prob}] Let $i^*$ be the largest integer such that there exists at least one tuple $(A_1,\ldots,A_d,w)$ in the data structure $\cal D$ in the $i^*$-th iteration such that $m_o(\dsubset) > \tau$. That is $\act_{i^*} > \tau$. For ease of analysis, let us define the two following events.
\begin{itemize}
\item $\cE_1:i^* \leq 2d \log n$.
\item $\cE_2:\est_{i^*}$ is a $(1 \pm \eps)$-approximation to $m_o(\cH)$.
\end{itemize}
Using the fact $\act_0=m_o(\cH) \leq n^d$ along with the Observation~\ref{lem:iter2}, we have $i^*\leq 2d\log n$ with probability at least $1-{2d \log n}\frac{2}{n^{5d}}$. That is $\pr(\cE_1) \geq 1-\frac{4d \log n}{n^{5d}}$.

Now let us condition on the event $\cE_1$. By the definition of $i^*$, we do the following in the $(i^*+1)$-th iteration. In Step 2, for each tuple $(\dsubset,w)$ present in $\cal D$, we determine $m_0(\dsubset)$ exactly, add it to $\Psi$ and remove $(\dsubset,w)$ from $\cal D$. Observe that $\act_{i^*+1}=0$, that is, $\est_{i^*+1}= \Psi_{i^* +1}=\est_{i^*}$. Since there are no tuples left in $\cal D$, we go to Step $1$. At the start of the $(i^*+2)$-th iteration, we report $\Psi_{i^* +1}=\est_{i^*}$ as the output. Using Observation~\ref{lem:iter1}, $\est_{i^*}$ is a ${(1 \pm \lambda)}^{i^*}$-approximation to $\est_0$ with probability at least $1-\frac{2d \log n}{n^{5d}}$. As $\est_0=m_o(\cH)$, $\lambda=\frac{\eps}{4d \log n}$, and $\cE_1$ has occurred, we have $\est_{i^*}$ is a $(1 \pm \eps)$-approximation to $m_o(\cH)$ with probability at least $1-\frac{2d\log n}{n^{3d+1}}$. That is $\pr(\cE_2~|~\cE_1) \geq 1-\frac{2d \log n}{n^{5d}}$.

Now, we analyze the query complexity of the algorithm on the conditional space that the events $\cE_1$ and $\cE_2$ have occurred. By the description of the algorithm, we make $\Oh_d\left(\frac{\log^{d+3}n}{\eps^2}\right)$ many \gonepis queries per tuple in Step $2$, and $\Oh_d(\log ^{d+1}n)$ many \gtwopis queries per tuple in Step $4$. Using Observation~\ref{obs:num_tuples}, there can be $\Oh_d\left( \frac{\log ^{4d} n}{\eps^2}\right)$ many tuples present in any iteration. Recall that the number of iterations is $(i^*+2)$, that is, $\Oh_d(\log n)$. Since $i^* \leq 2d \log n$, the query complexity of our algorithm is $\Oh_d \left(\log n \cdot \frac{\log ^{4d} n}{\eps^2} \cdot \left( \frac{\log^{d+3}n}{\eps^2} +\log^{d+1} n\right) \right)=\Oh_d\left( \frac{\log ^{5d+4} n}{\eps^4}\right)$, where each query is either a \gonepis or a \gtwopis query.

Now we compute the probability of success of our algorithm. Observe that
\begin{center}
$\pr(\mbox{{\sc Success}}) \geq \pr(\cE_1 \cap \cE_2)
= \pr(\cE_1) \cdot \pr(\cE_2~|~\cE_1) 
\geq \left(1-\frac{4d \log n}{n^{5d}}\right) \cdot \left(1-\frac{2d \log n}{n^{5d}}\right) 
 \geq 1-\frac{1}{n^{4d}}
$
\end{center}

\end{proof}



==> exact.tex <==
\section{Proof of Lemma for Exact Estimation} \label{sec:exact}

\noindent In this Section, we prove Lemma~\ref{lem:exact}. We restate the lemma for easy reference.

\begin{lem} [Exact Estimation: Lemma~\ref{lem:exact} restated] \label{lem:exact1} There exists a deterministic algorithm $\cAe$ that takes as input --- a $d$-uniform hypergraph $\cH$, constants $a_1,\ldots,a_s \in [d]$ such that $\sum_{i=1}^s a_i =d$ where $s \in [d]$, pairwise disjoint subsets $A_1,\ldots,A_s$ of $U(\cH)$, and threshold parameter $\tau \in \N$ --- and decides whether {the number of ordered hyperedges} $m_o(\ssubset) \leq \tau$ using $\cO_d(\tau \log n)$ \gonepis queries. Moreover, the algorithm finds the exact value of $m_o(\ssubset)$ when $m_o(\ssubset) \leq \tau$. 
\end{lem}

\begin{algorithm}[!ht]
%\scriptsize

\SetAlgoLined

\caption{{$\cAe$($\dsubset,\tau$)}}
\label{algo:exact}
\KwIn{Subsets $A_1,\ldots, A_d$ of vertex set $U(\cH)$ of a $d$-uniform hypergraph $\cH$ and a threshold $\tau$.}
\KwOut{Check if $m_o(\ssubset) \leq \tau$. If Yes, return the exact value of $m_o(\ssubset)$.}
%\LinesNumbered

Initialize a tree ${\cal T}$ with $(\ssubset)$ as the root and label the root with $1$.\\
\If{the number of nodes in $\cT$ is more than $2^{d+2} \tau \log n$ }
{
Report that $m_o(\ssubset) > \tau$ as the output.
}
\While{there is a leaf node $m_o(\tsubset)$ in the tree with label $1$}
{
{Note that $0 \leq b_i \leq d$ and $\sum\limits_{i=1}^t b_i = d$. Also, for $i \neq j$, either $B_i \cap B_j = \emptyset$ or $B_i=B_j$.}\\
\If{ $m_o(\tsubset)=0$ or there exists an $i \in [t]$ such that $\size{B_i} < b_i$}
{ 
Label $(\tsubset)$ with $0$.
}
\Else
{
Label $(\tsubset)$ with $1$.\\
Partition each $B_i$ into two parts $B_{i1}$ and $B_{i2}$ such that $\size{B_{i1}}=\lceil \frac{B_{i}}{2} \rceil$ and $\size{B_{i2}}=\lfloor \frac{B_{i}}{2} \rfloor$. \\
Add nodes of the form $(C_{11j},\ldots,C_{1b_1j}, \ldots, C_{t1j},\ldots,C_{tb_tj})$ as children of $(\tsubset)$ and label them 1, for $j\in \{1,2\}$, where $C_{ib_i1}=\lceil \frac{C_{ib_i}}{2}\rceil$ and $C_{ib_i2}=\lfloor \frac{C_{ib_i}}{2}\rfloor$.
}
}
Generate $\cT'$ as the tree after deleting all the leaf nodes in $\cT$.\\
Report the number of leafs in $\cT'$ as $m_o(\ssubset)$ as the output.
\end{algorithm}


\begin{proof} First, we discuss an algorithm that determines the exact value of $m_o(\ssubset)$ using $\Oh_d(m_o(\ssubset) \log n)$ \gonepis queries. Then, we argue how to modify it to obtain the desired bound.  {We initialize a multi-ary  tree ${\cal T}$ with $(\ssubset)$ as the root and then build it level by level. At the next level, each $A_i$ is split into two halves -- $A_{i,1}$ and $A_{i,2}$ and each node in the next level is labeled with $A_{i,j}$, $i \in \{1, \ldots,s\}$, $j \in \{1,2\}$; so in the next level there are $2^s \leq 2^d$ nodes. Notice that as we go down the levels in ${\cal T}$, each node corresponds to \gonepis queries with smaller and smaller sets. }  
The nodes of the tree are labeled with either $0$ or $1$. If $m_o(\ssubset)=0$, we label the root with $0$ and terminate. Otherwise, we label the root {(node)} with $1$ and keep branching, and as long as there is a leaf node $(B_1^{[b_1]},\ldots,B_{t}^{[b_t]})$ {in this branch} labeled with $1$, we do the following. Note that $0 \leq b_i \leq d$ and $\sum\limits_{i=1}^t b_i = d$. Also, for $i \neq j$, either $B_i \cap B_j = \emptyset$ or $B_i=B_j$ {because it is a tree-based disjoint partitioning}.

\begin{itemize}
	\item[(i)] If $m_o(\tsubset)=0$ or there exists an $i \in [t]$ such that $\size{B_i} < b_i$, then we label $(\tsubset)$ with $0$. Otherwise, we label $(\tsubset)$ with $1$.
	\item[(ii)] We partition each $B_i$ into two parts $B_{i1}$ and $B_{i2}$ such that $\size{B_{i1}}=\lceil \frac{B_{i}}{2} \rceil$ and $\size{B_{i2}}=\lfloor \frac{B_{i}}{2} \rfloor$. There may exist some $B_i$ for which $B_{i2}=\emptyset$. We add nodes of the form $(\underbrace{C_{11j},\ldots,C_{1b_1j}}, \ldots, \underbrace{C_{t1j},\ldots,C_{tb_tj}})$ as the children of $(\tsubset)$ and label them 1, for $j\in \{1,2\}$ where $C_{ib_i1}=\lceil \frac{C_{ib_i}}{2}\rceil$ and $C_{ib_i2}=\lfloor \frac{C_{ib_i}}{2}\rfloor$. Note that for each node $(\tsubset)$ with label $1$, we add $\prod\limits_{i=1}^{t} 2^{b_i} = 2^d$ nodes as children of it.
\end{itemize}

Note that the algorithm stops when all the leaf nodes of tree $\cT$ are labeled with $0$. Let $\cT'$ be the tree after deleting all the leaf nodes in $\cT$. %\complain{(Gopi, nodes corresponding to $m_o(\cdot) = 0$, where the branching stopped, are also leaves. What do we do with them?)} 
Observe that $m_o(\tsubset)$ is the number of leaf nodes in $\cT'$ and
\begin{itemize}
	\item the height of ${\cal T}$ is bounded by $\log \left(\max\limits_{i \in [t]} \size{A_i}\right) +1  \leq \log n +1 $. %({\bf should it be $\log$ of $\max$?})
	\item the query complexity of the above procedure is bounded by the number of nodes in ${\cal T}$ as we make at most one query per node of $\cT$.
\end{itemize}



The number of nodes in $\cT'$ which equals the number of internal nodes of $\cT$ is bounded by $(\log n+1) \cdot m_o(\tsubset)$. Hence, the number of leaf nodes in $\cT$ is at most $2^d (\log n + 1) \cdot m_o(\ssubset)$. The total number of nodes in $\cT$ is at most $(2^d+1) (\log n+1) \cdot m_o(\ssubset) \leq 2^{d+2} \cdot m_o(\ssubset) \log n$. Putting everything together the number of \gonepis queries made by our algorithm is at most $ 2^{d+2} \cdot m_o(\ssubset) \log n$.
 
The algorithm, as claimed in the statement of Lemma~\ref{lem:exact1}, proceeds similar to the one presented above by initializing a tree $\cT$ with $(\ssubset)$ as the root. If $m_o(\ssubset) \leq \tau$, then we can find the exact value of $m_o(\ssubset)$ using at most $2^{d+2} \tau \log n$ \gonepis queries and the number of nodes in $\cT$ is bounded by $ 2^{d+2} \tau \log n$. So, if the number of nodes in $\cT$ is more than $2^{d+2} \cdot  m_o(\ssubset) \log n$ at any instance during the execution of the algorithm, we report $m_o(\ssubset) >\tau$ and terminate. Hence, our algorithm makes $\Oh_d(\tau \log n)$ many \gonepis queries, decides whether $m_o(\ssubset) \leq \tau$, and determines the exact value of $m_o(\ssubset)$ in the case $m_o(\ssubset) \leq \tau$. 
\end{proof}


==> overview.tex <==


\remove{\comments{In subset size estimation problem using subset query oracle, we want to estimate the size of a subset $S\subseteq T$ using an oracle which tells us, given a query set $Q\subseteq T$, whether $Q \cap T$ is empty or not. Viewed differently, this is about estimating an unknown set $S$ by looking at its intersection pattern with a known set $T$.}

The hyperedge estimation problem can be thought of as a generalized version of the subset size estimation problem. We show using an induction on $d$ that \hest using \gpis queries in a $d$-uniform hypergraph generalizes from the subset size estimation problem.}


\subsection{Our work in a nutshell}
\begin{figure}[h!]
	\centering
	\includegraphics[width=\linewidth]{flowchart}
	\caption{Flow chart of the algorithm. The highlighted texts indicate the basic building blocks of the algorithm. We also indicate the corresponding lemmas that support the building blocks. The building blocks marked with {\Large $\star$} correspond to the steps that make queries.} %\complain{Gopi: Correct the lemma numbers later. Also, can we highlight which query is used in which building block?}
	\label{fig:flowchart}
\end{figure}

\paragraph{The algorithmic framework} In Figure~\ref{fig:flowchart}, we give a flowchart of the algorithm. Our algorithm begins by adding the $d$-partite hypergraph $\cH(U^{[d]})$ in a suitable data structure, let us call it $\cD$. For each hypergraph in $\cD$, using the \emph{exact estimation} process, we \emph{exactly count} the number of hyperedges in a hypergraph if the number of hyperedges is less than a \emph{threshold} $\tau$ and remove the corresponding hypergraph from $\cal D$. For hypergraphs in which the number of hyperedges is more than $\tau$, we can not do \emph{exact estimation}. So, we resort to \emph{sparsification} if the number of  hypergraphs left in $\cD$ is not \emph{large}, i.e., below a \emph{threshold} $\cN$. Hypergraph sparsification breaks a $d$-partite hypergraph into a disjoint union of $d$-partite sub-hypergraphs. As sparsification goes on in iterations, it may populate the data structure $\cD$ with \emph{significantly many} hypergraphs. In that case, we do a \emph{coarse estimation} followed by \emph{sampling} to have a reasonable number of sub-hypergraphs and then go back to the exact estimation step and continue in a loop. \gonepis and \gtwopis queries will be used for exact and coarse estimations, respectively; their logarithmic equivalence with \gpis will prove the final result. For ease of analysis, we consider {\it ordered} hyperedges. Fact \ref{obs:1} relates $m(A_1,\ldots,A_d)$ and $m_o(A_1,\ldots,A_d)$, the number of unordered and ordered hyperedges, respectively. 
\remove{
Since \gonepis and \gtwopis queries can be simulated using at most logarithmic \gpis queries, in the description of our algorithm, we use \gonepis and \gtwopis queries interchangeably, the usage of the particular query would be clear from the context. For ease of analysis we consider {\it ordered} hyperedges. The relation between the number of unordered hyperedges $m(A_1,\ldots,A_d)$ and the number of ordered hyperedges $m_o(A_1,\ldots,A_d)$ in sets $A_1,\ldots,A_d$ is given as Fact \ref{obs:1}.
}

\remove{
\paragraph{Exact estimation.} In this step, we look at a $d$-partite sub-hypergraph and decide whether $m_o(U^{[d]})$, the number of ordered hyperedges, is larger or smaller than a threshold $\tau$~\footnote{Threshold $\tau$ will be fixed later in Section~\ref{sec:exact}.}, and if $m_o(U^{[d]}) \leq \tau$, compute the exact value of $m_o(U^{[d]})$ using Lemma~\ref{lem:exact}, whose proof is in Section~\ref{sec:exact}. If $m_o(U^{[d]})$ is greater than $\tau$ \complain{and the number of hypergraphs in $\cD$ is below a threshold}, we move to the sparsification step, else to the coarse estimation step.  \comments{Gopi:Can we change this paragraph a bit as follows?}
}

\paragraph{Exact estimation.} In this step, we look at a $d$-partite sub-hypergraph $\cH(\ssubset)$ and decide whether $m_o(\ssubset)$, the number of ordered hyperedges, is larger or smaller than a threshold $\tau$~\footnote{Threshold $\tau$ will be fixed later in Section~\ref{sec:exact}.}, and if $m_o(\ssubset) \leq \tau$, compute the exact value of $m_o(\ssubset)$ using Lemma~\ref{lem:exact}, whose proof is in Section~\ref{sec:exact}, and then delete it from $\cD$. If the number of hypergraphs in $\cD$ is below the threshold $\cN$, with the number of ordered hyperedges in it more than $\tau$, we move to the sparsification step, else to the coarse estimation step. 


\begin{lem} [Exact Estimation] \label{lem:exact} There exists a deterministic algorithm $\cAe$ that takes as input --- a $d$-uniform hypergraph $\cH$, constants $a_1,\ldots,a_s \in [d]$ such that $\sum_{i=1}^s a_i =d$ where $s \in [d]$, pairwise disjoint subsets $A_1,\ldots,A_s$ of $U(\cH)$, and a threshold parameter $\tau \in \N$ --- and decides whether the number of ordered hyperedges $m_o(\ssubset) \leq \tau$ using $\cO_d(\tau \log n)$ \gonepis queries. Moreover, $\cAe$ finds the exact value of $m_o(\ssubset)$ when $m_o(\ssubset) \leq \tau$. \end{lem}

\paragraph{Sparsification.} 
We {\sc color} $U(\cH)$, the vertices of hypergraph, with $[k]$ colors to sparsify the $d$-partite hypergraph $\cH(U^{[d]})$ so that 
\begin{itemize}
	\item[(i)] the sparsified hypergraph consists of a set of $d$-partite sub-hypergraphs and  
	\item[(ii)] a proper scaling of the sum of the number of ordered hyperedges in the sub-hypergraphs is a \emph{good} estimate of $m_o(U^{[d]}),U=U(\cH),$ with high probability. 
\end{itemize}
The sparsification result is formally stated next. The proof uses the \emph{method of averaged bounded differences} and \emph{Chernoff-Hoeffding} inequality. The detailed proof is given in Section~\ref{sec:sparse}. The heart of our work is the general sparsification routine that we believe will find independent uses. 
\begin{lem}[Sparsification] \label{lem:sparse}
Let $\cH$ be any $d$-uniform hypergraph and $k\geq 1$ be any positive integer. Let
        \begin{itemize}
                \item $h_d:[k]^d\rightarrow \{0,1\}$ be a hash function such that independently for any $d$-tuple ${\bf a}\in [k]^d$, $\pr[h_d({\bf a})=1]=\frac{1}{k}$.
                \item $A_1,\ldots,A_s$ be any pairwise disjoint subsets of the vertex set $U(\cH)$, where $1\leq s\leq d$. Let us choose any $a_i\in [d]$ vertices from $A_i$ such that $\sum_{i=1}^s a_i=d$. 
                \item Vertices in $A=\bigcup_{i=1}^s A_i$ are \colored with $[k]$. $\chi(i,j)$'s denote the color classes for each $A_i$, that is, $\chi(i,j)=\{v\in A_i:~v~\mbox{is {\colored} with color $j$}\}$, where $i \in [s]$ and $j \in [k]$. 
                \item An ordered hyperedge $(x_1,\ldots,x_d)$ is said to be \emph{properly colored} if $h_d(c_1,\ldots,c_d)=1$ where $c_i$ is the color of $x_i$. Let $\cR_d$ denote the number of \emph{properly colored} hyperedges defined as follows. $$\cR_d=\sum\limits_{(c_1,\ldots,c_d) \in [k]^d} m_o\left( \underbrace{\chi({1,c_1}),\ldots,\chi({1,c_{a_1}})}_{\mbox{color classes for } A_1^{[a_1]}}, \ldots, \underbrace{\chi({s,c_{d-a_s+1}}),\ldots,\chi({s,c_{d}}}_{\mbox{color classes for } A_s^{[a_s]}}) \right) \times h_d(c_1,\ldots,c_d).$$
        \end{itemize}
Then, for a suitable constant $\theta > d$ and $p_d = \frac{d!}{n^{4\theta -2d}}$,
$$ \pr \left(\size{ \cR_d  - \frac{m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})}{k}} \geq 2^{2d}\theta^d   \sqrt{ d! ~ m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]}) \log^d n} \right) \leq p_d.$$
\end{lem}
Sparsification ensures that $m_o(U^{[d]})$, the number of ordered hyperedges between $A_1^{[a_1]},\ldots,A_s^{[a_s]}$, is approximately preserved when $m_o(U^{[d]})$ is above a threshold $\tau$.  

%%%%%%%%%%%%%%%%%%%%
Assume that $m_o(U^{[d]})$ is \emph{large}~\footnote{{A fixed polylogarithmic quantity to be decided later in Section~\ref{sec:algo}.}} and $\cH(U^{[d]})$ has been sparsified. We add to the data structure $\cD$ a set of $d$-partite sub-hypergraphs obtained from the sparsification step. Refer to the flowchart in Figure~\ref{fig:flowchart} again. With the new $d$-partite sub-hypergraphs, we loop back to the exact estimation step. 
\remove{
For each $d$-partite hypergraph $\cH(\ssubset)$ in the data structure, we check whether $m_o(\ssubset)$ is less than the threshold $\tau$ using the above algorithm for exact estimation (Lemma~\ref{lem:exact}). If it is less than threshold $\tau$, we compute the exact value of $m_o(\ssubset)$ using Lemma~\ref{lem:exact} and remove $\cH(\ssubset)$ from the data structure. 
}
After the exact estimation step, we are left with some $d$-partite hypergraphs such that the number of ordered hyperedges in each hypergraph is more than the threshold $\tau$. If the number of such hypergraphs {present in $\cD$} is not large, i.e., below $\cN$, then we sparsify each hypergraph $\cH(\ssubset)$ using the algorithm corresponding to Lemma~\ref{lem:sparse}.  
\remove{ such that
\begin{itemize}
	\item[(i)] we obtain some $d$-partite sub-hypergraphs for each of the sparsified hypergraphs, and 
	\item[(ii)] a constant scaling of the sum of the number of ordered hyperedges in the sparsified sub-hypergraphs approximates $m_o(\ssubset)$.
\end{itemize}
Gopi: This (i) and (ii) was written at the beginning also. Do we need it again? \comments{Yes, we can remove the above red marked text.}
}

\paragraph{Coarse estimation and sampling.} If we have a large number of $d$-partite sub-hypergraphs of $\cH(U^{[d]})$ and each sub-hypergraph contains a large number of ordered hyperedges, then we \emph{coarsely} estimate the number of ordered hyperedges in each sub-hypergraph; see Figure~\ref{fig:flowchart}. Our estimator is correct up to a $\Oh_d(\log^{d-1} n)$ factor using the algorithm corresponding to the following lemma, whose proof is given in Section~\ref{sec:coarse}. 
\begin{lem}[Coarse Estimation] \label{lem:coarse_main} There exists an algorithm $\cAc$ that takes as input $d$ subsets $A_1,\ldots, A_d$ of vertex set $U(\cH)$ of a $d$-uniform hypergraph $\cH$ and returns $\hat{E}$ as an estimate for $m_o(\dsubset)$ such that 
	$$ \frac{m_o(\dsubset)}{8d^{d-1}2^d \log^{d-1} n} \leq \hat{E} \leq 20d^{d-1}2^d \cdot m_o(\dsubset) \log^{d-1} n $$
with probability at least $1-n^{-8d}$. Moreover, the number of \gtwopis queries made by the algorithm is $\Oh_d(\log ^{d+1} n)$. \end{lem} 

First, we coarsely estimate the number of ordered hyperedges in each sub-hypergraph. Then we sample a set of sub-hypergraphs such that a weighted sum of the number of hyperedges in the sample approximately preserves the sum of the number of ordered hyperedges in the sub-hypergraphs. This kind of sampling technique, also known as the importance sampling, is given for the edge estimation problem by Beame~\etal~\cite{BeameHRRS18}. The lemma corresponding to this sampling technique is formally stated as Lemma~\ref{lem:importance1} in Appendix~\ref{sec:prelim}. The importance sampling lemma that we require is stated as follows. 

\begin{lem}[Importance Sampling] \label{lem:importance-app-over} 
Let $\{(A_{i1},\ldots,A_{id},w_i):i \in [r]\}$ be the set of tuples in the data structure $\cD$ and $e_i$ be the coarse estimate for $m_o(A_{i1},\ldots,A_{id},w_i)$ such that (i) $w_i,e_i \geq 1~ \forall i \in [r]$, (ii) $\frac{e_i}{\alpha} \leq m_o(A_{i1},\ldots,A_{id}) \leq e_i \cdot \alpha$ for some $\alpha >0$ and $\forall ~i \in [r]$, and (iii) $\sum_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})} \leq M$. Then, there exists an algorithm that finds a set $\{(A'_{i1},\ldots,A'_{id},w'_i):i \in [r']\}$ of tuples, with probability at least $1-\delta$, such that the above three conditions hold and 
\begin{equation*}
%\begin{center}
\size{\sum_{i=1}^{r'} {w'_i\cdot m_o(A'_{i1},\ldots,A'_{id})}-\sum_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})}} \leq \lambda S \, , 
\end{equation*}
%\end{center}
where $S=\sum_{i=1}^r {w_i m_o(A_{i1},\ldots,A_{id})}$, $\lambda>0$, $\delta >0$ and $r'=\cO\left(\frac {\alpha^4 \log M}{\lambda^{2}} \left(\log \log M + \log \frac{1}{\delta}\right)\right)$. 
\end{lem}

\paragraph{Putting things together.} The data structure $\cal D$ that our iterative algorithm uses (see the flowchart in Figure~\ref{fig:flowchart}) has an accumulator $\Psi$ for the number of hyperedges and a set of tuples representing the $d$-partite sub-hypergraphs along with their weights -- these $d$-partite sub-hypergraphs are generated from sparsification. The algorithm uses the \emph{exact estimation} step (viz. Algorithm~\ref{algo:exact}) to figure out if the number of hyperedges $m_o(\dsubset) \leq \tau$ using Lemma~\ref{lem:exact}. If $m_o(\dsubset) \leq \tau$, we add $w \cdot m_o(\dsubset)$ to $\Psi$ and remove the tuple $(A_1,\ldots,A_d,w)$ from $\cal D$. If the number of tuples in $\cal D$ is at most $\cN = \kappa_d \cdot \frac{\log ^{4d} n}{\eps^2}$, then we carry out a sparsification step, else we do an importance sampling; a coarse estimation step (viz. Algorithms~\ref{algo:verify} and~\ref{algo:coarse}) acts as a pre-processing step for importance sampling. We do either sparsification or coarse estimation followed by importance sampling in an iteration because their roles are complementary. While successive sparsifications ease estimating the number of hyperedges by breaking a $d$-partite hypergraph into a disjoint union of $d$-partite sub-hypergraphs, the number of such $d$-partite sub-hypergraphs may be as high as $4^d \cdot \cN =4^d \kappa_d \cdot \frac{\log ^{4d} n}{\eps^2}$ (see Observation~\ref{obs:num_tuples}). Coarse estimation followed by importance sampling (see Lemma~\ref{lem:importance-app-over}) ensures that the effect of sparsification is neutralized so that the number of tuples in $\cal D$ is at most $\cN$. This ensures that out of two successive iterations of the algorithm, there is at least one sparsification step. The coarse estimation applies when the number of tuples $r>\cN=\frac{\kappa_d\log^{4d} n}{\eps^2}$. 
\remove{For each tuple in $\cal D$, we find an estimate $\hat{E_i}$ such that $\frac{m_o(A_1,\ldots,A_d)}{\alpha} \leq \hat{E_i} \leq \alpha m_o(A_1,\ldots,A_d)$ using $\Oh_d(\log^{d+1} n)$ \gtwopis queries per tuple (see Lemma~\ref{lem:coarse_main} for the precise value of $\alpha$).}
For each tuple in $\cal D$, we find an estimate $\hat{E_i}$ using $\Oh_d(\log^{d+1} n)$ \gtwopis queries per tuple (see Lemma~\ref{lem:coarse_main}).
This estimate serves as condition (ii) for the application of Lemma~\ref{lem:importance-app-over}. 
\remove{For the $r$ tuples in $\cal D$, let $e_i$ be the coarse estimate of $m_o(A_{i1},\ldots,A_{id},w_i)$, $i \in [r]$, such that (i) $w_i,e_i \geq 1~ \forall i \in [r]$, (ii) $\frac{e_i}{\alpha} \leq m_o(A_{i1},\ldots,A_{id}) \leq e_i \cdot \alpha$ for some $\alpha >0$ and $\forall ~i \in [r]$, and (iii) $\sum_{i=1}^r {w_i\cdot m_o(A_{i1},\ldots,A_{id})} \leq M$.} Because of the importance sampling (see Lemma~\ref{lem:importance-app-over}), one can replace the $r$ tuples in $\cal D$ with a sample of $r'$ tuples such that the required estimate is approximately maintained. Since $r' \leq \kappa_d \cdot \frac{\log^ {4d} n}{\eps^2}=\cN$, the next step will be sparsification.

Observe that the query complexity of each iteration is polylogarithmic. Note that the number of ordered hyperedges reduces by a constant factor after each sparsification step. So, the number of iterations is bounded by $\Oh_d(\log n)$. Hence, the query complexity of our algorithm is polylogarithmic. This completes a high level description of our algorithm. 

\remove{
Using the sampling scheme mentioned above, we check whether $m_o(\ssubset)$ is less than threshold $\tau$ using Lemma~\ref{lem:exact} for each $d$-partite hypergraph $\cH(\ssubset)$. If $m_o(\ssubset)<\tau$, we compute the exact value of $m_o(\ssubset)$ using Lemma~\ref{lem:exact} and remove $\cH(\ssubset)$ from the data structure. Otherwise, we perform sparsification, exact counting and coarse estimation to estimate $m_o(\ssubset)$. Observe that the query complexity of each iteration is polylogarithmic. Note that the number of ordered hyperedges reduces by a constant factor after each sparsification step. So, the number of iterations is bounded by $\Oh_d(\log n)$. Hence, the query complexity of our algorithm is polylogarithmic. This completes a high level description of our algorithm. 
}

\subsection{Our work vis-a-vis some recent works} \label{sec:compare}

\paragraph*{Comparison with Beame et al.~\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}:}
Beame et al.~\cite{BeameHRRS18} showed that {\sc Edge Estimation} problem can be solved using $\Oh(\eps^{-4}\log ^{14} n)$ many \bis queries. Note that a \bis query is a special case of \gpis query for $d=2$. Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} first considered the {\sc Triangle Estimation} problem in graphs using a \tis query oracle, a generalization of \bis query oracle. \remove{As a first step towards the generalization of {\sc Edge Estimation} using \bis towards \hest using \gpis, Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} considered {\sc Triangle Estimation} in graphs using a query oracle called \tis.} They showed that an $(1 \pm \eps)$-approximation to the number of triangles can be found by using $\Oh(\Delta^{12} \eps^{-12} \log ^{25} n)$ many \tis queries, where $\Delta$ denotes the maximum number of triangles sharing an edge. Note that the {\sc Triangle Estimation} problem in graphs using \tis queries is analogous to the \hest problem in $3$-uniform hypergraphs using a special \gpis query when $d=3$. In this paper, we build on the works of Beame et al.~\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} for \hest using \gpis queries. Our main contribution in this work is twofold and that answers Questions 1 and 2 posed in Section~\ref{sec:intro}. Firstly, our query complexity bounds are independent of $\Delta$, this dependence on $\Delta$ was present in the work of Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. 
Secondly, our work can be seen as a complete generalization of the works of Beame et al.\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} to $d$-uniform hypergraphs. \remove{Secondly, our query complexity bounds are independent of $\Delta$, this dependence on $\Delta$ was present in the work of Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. Our results not only remove the dependency on $\Delta$ present in the work of Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}, but also generalizes the results of Beame et al.\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} to $d$-uniform hypergraph setting} As mentioned earlier, the extension from the {\sc Edge Estimation} problem using \bis queries to the {\sc Hyperedge Estimation} problem using \gpis queries is not obvious as edges in a graph can intersect in at most one vertex, but the intersection pattern of hyperedges in hypergraphs is complicated. The main building blocks of the algorithms of Beame {\it{et al.}} and Bhattacharya {\it{et al.}} are \emph{sparsification}, \emph{exact estimation} and \emph{coarse estimation}. We generalize their exact estimation and coarse estimation algorithms by more detailed and careful analysis. The sparsification algorithm in the work of Beame et al.~\cite{BeameHRRS18} uses heavily the fact that two edges in a graph can intersect with at most one vertex. This may be the reason why Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC} required a bound on the number of triangles sharing an edge. In this paper, we show that an ingenious way of coloring the hyperedges in a $d$-uniform hypergraph and an involved use of induction on $d$ generalize the results of both Beame et al.~\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. The main technical and non-trivial contribution in this paper is the sparsification algorithm, which enables us to generalize the works of Beame et al.~\cite{BeameHRRS18} and Bhattacharya et al.~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. Their sparsification results do not generalize for arbitrary $d$ without any assumptions on the intersection pattern of the hyperedges.  



\paragraph*{Comparison with Dell et al.~\cite{DellLM19}:} Concurrently and independently, Dell et al.~\cite{DellLM19} obtained similar results for the hyperedge estimation problem. They showed that one can find an $(1 \pm \eps)$-approximation to the number of hyperedges in a $d$-uniform hypergraph by using $\Oh_d\left(\frac{\log ^{4d+7} n}{\eps^2} \log \frac{1}{\delta}\right)$ \emph{colorful independent set} queries with probability at least $1-\delta$. A colorful independent set query is same as that of a \gpis query oracle considered in this paper; \gpis{} query was introduced by Bishnu et al.~\cite{BishnuGKM018,Bishnu18}. Note that the algorithm of Dell et al.~\cite{DellLM19} for \hest uses comparable but fewer number of \gpis queries. However, our algorithm is different and conceptually much simpler than that of Dell et al.~\cite{DellLM19}. Most importantly, the main technical tool, our sparsification step is completely different from theirs.

\remove{
\subsection{{The role of the hash function in sparsification}}

\noindent We feel our work could generalize the framework of Beame et al.~\cite{BeameHRRS18} to hyperedge estimation mainly because of the new sparsification result aided by an involved use of induction. The sparsification result depends on the particular choice of hash function. As we move from edge to triangle and then to hyperedge in a $d$-uniform hypergraph, implicit structure blow up, and managing their interrelations also become difficult. Consider the following. Two edges can intersect in at most one vertex. two triangles can intersect in at most two vertices and two hyperedges in $d$-uniform hypergraph intersect in at most $d-1$ vertices. \remove{The existence of three triangles $(a,b,x)$, $(b,c,y)$ and $(a,c,z)$ in $G$ imply the existence of the triangle $(a,b,c)$ in $G$. The number of such implicit structures will blow up for hyperedges.}

To count the number of edges in $G$, Beame et al.~\cite{BeameHRRS18} sparsify the graph by coloring the vertices with $k$ colors and looking at the edges between certain pair of color classes. So, it boils down to counting the number of properly colored edges. This random coloring process can be encoded by the hash function $h:[k]\rightarrow [k]$. In our first effort in generalizing this work to count the number of triangles in a graph, we extended the above hash function to the following one -- $h:[k] \times [k] \rightarrow [k]$ in ~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. Look at any edge $(a,b)$ in this graph under the above hash function. The edge is properly colored if the colors on the vertices of the edge come from specified color classes. We count all triangles on these properly colored edges, and scale it appropriately. Once an edge is not properly colored, we may miss it and hence, all triangles incident on that edge. This is why we need a bound on the number of triangles incident on an edge in~\cite{Bhatta-abs-1808-00691,BhattaISAAC}, otherwise the variance blows up and the concentration inequality gives poor result.

In this work, we consider a different hashing scheme with the hash function $h:[k]^d \rightarrow \{0,1\}$, in the $d$-uniform hypergraph setting, with a suitable probability of hash values becoming $1$. So, for triangles ($3$-uniform hypergraph), the particular hash function is $h:[k]^3 \rightarrow \{0,1\}$. So, there is no concept of proper and improper edge. All edges are taken into consideration and then all triangles, and we can work with any number of triangles incident on an edge. Moreover, there is an inductive nature to this particular choice of hash function. Consider fixing the color of a vertex of a triangle. Then the hash function $h : [k]\times[k]\rightarrow \{0,1\}$ behaves as a random coloring on the other two vertices of the triangle.
}

==> sparse.tex <==
\section{Sparsification: Proof of Lemma~\ref{lem:sparse}} \label{sec:sparse}
\noindent
We start by reproducing the statement of the Lemma~\ref{lem:sparse} below. Sparsification ensures that the number of ordered hyperedges $m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})$ is approximately preserved across any pairwise disjoint subsets of vertices $A_1,\ldots,A_s$ and integers $a_1,\ldots,a_s$ such that $\sum_{i=1}^s a_i=d$.

\begin{lem}[Sparsification] \label{lem:sparse2}
Let $\cH$ be any $d$-uniform hypergraph and $k\geq 1$ be any positive integer. Let
	\begin{itemize}
		\item $h_d:[k]^d\rightarrow \{0,1\}$ be a hash function such that independently for any tuple ${\bf a}\in [k]^d$, $$\pr[h_d({\bf a})=1]=\frac{1}{k}.$$
		\item $A_1,\ldots, A_s$ be any pairwise disjoint subsets of $U(\cH)$, where $1\leq s\leq d$. Let us choose any $a_i \in [d]$ vertices from $A_i$ such that $\sum_{i=1}^s a_i=d$. 
		\item Vertices in $A=\bigcup_{i=1}^s A_i$ are \colored with $[k]$. $\chi(i,j)$'s denote the color classes for each $A_i$, that is, $\chi(i,j)=\{v\in A_i:~v~\mbox{is \colored with color $j$}\}$, where $i \in [s]$ and $j \in [k]$. \remove{Vertices in $A=\cup A_i$ be \colored with $[k]$, where the color classes in $A_i$ is denoted as $\chi(i,j)=\{v\in A_i:~v~\mbox{is colored with color $j$}\}$, where $i \in [s]$ and $j \in [k]$.}
		\item An ordered hyperedge $(x_1,\ldots,x_d)$ is said to be \emph{properly colored} if $h_d(c_1,\ldots,c_d)=1$ where $c_i$ is the color of $x_i$. Let $\cR_d$ denote the number of \emph{properly colored} hyperedges defined as follows. $$\cR_d=\sum\limits_{(c_1,\ldots,c_d) \in [k]^d} m_o\left( \underbrace{\chi({1,c_1}),\ldots,\chi({1,c_{a_1}})}_{\mbox{color classes for } A_1^{[a_1]}}, \ldots, \underbrace{\chi({s,c_{d-a_s+1}}),\ldots,\chi({s,c_{d}}}_{\mbox{color classes for } A_s^{[a_s]}}) \right) \times h_d(c_1,\ldots,c_d).$$
	\end{itemize}   
Then, for a suitable constant $\theta > d$ and $p_d = \frac{d!}{n^{4\theta -2d}}$,
$$ \pr \left(\size{ \cR_d  - \frac{m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})}{k}} \geq 2^{2d}\theta^d   \sqrt{ d! m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]}) \log^d n} \right) \leq p_d.$$
\end{lem}
The above lemma says that the properly colored hyperedges approximate the number of ordered hyperedges upto a scaling factor when the number of (ordered) hyperedges is above a thershold.
Before getting into the formal proof of the lemma, let us explore the role of the hash function in sparsification. 

\subsection{{The role of the hash function in sparsification}}
\noindent 
We feel our work could generalize the framework of Beame et al.~\cite{BeameHRRS18} to hyperedge estimation mainly because of the new sparsification result aided by an involved use of induction. The sparsification result depends on the particular choice of hash function. As we move from edge to triangle and then to hyperedge in a $d$-uniform hypergraph, implicit structures blow up, and managing their interrelations also become difficult. Consider the following. Two edges can intersect in at most one vertex. two triangles can intersect in at most two vertices and two hyperedges in $d$-uniform hypergraph intersect in at most $d-1$ vertices. \remove{The existence of three triangles $(a,b,x)$, $(b,c,y)$ and $(a,c,z)$ in $G$ imply the existence of the triangle $(a,b,c)$ in $G$. The number of such implicit structures will blow up for hyperedges.}

To count the number of edges in $G$ using sparsification, Beame et al.~\cite{BeameHRRS18} \colored the vertices with $k$ colors and looked at the edges between certain pair of color classes. So, it boils down to counting the number of properly colored edges. This random coloring process can be encoded by the hash function $h:[k]\rightarrow [k]$. In our first effort in generalizing this work to count the number of triangles in a graph, we extended the above hash function to the following one -- $h:[k] \times [k] \rightarrow [k]$ in ~\cite{Bhatta-abs-1808-00691,BhattaISAAC}. Look at any edge $(a,b)$ in this graph under the above hash function. The edge is properly colored if the colors on the vertices of the edge come from specified color classes. We count all triangles on these properly colored edges, and scale it appropriately. Once an edge is not properly colored, we may miss it and hence, all triangles incident on that edge. This is why we need a bound on the number of triangles incident on an edge in~\cite{Bhatta-abs-1808-00691,BhattaISAAC}, otherwise the variance blows up and the concentration inequality gives poor result.

In this work, we consider a different hashing scheme with the hash function $h:[k]^d \rightarrow \{0,1\}$, in the $d$-uniform hypergraph setting, with a suitable probability of hash values becoming $1$. For triangles ($3$-uniform hypergraph), the particular hash function is thus $h:[k]^3 \rightarrow \{0,1\}$. So, there is no concept of proper and improper edges. All edges are taken into consideration and then all triangles, and we can work with any number of triangles incident on an edge. Moreover, there is an inductive nature to this particular choice of hash function. Consider fixing the color of a vertex of a triangle. Then the hash function $h : [k]\times[k]\rightarrow \{0,1\}$ behaves as a random coloring on the other two vertices of the triangle. 

%\comments{
To elaborate further, our sparsification algorithm independently colors the vertices of the hypergraph by selecting a color uniformly at random from $\{1, \ldots, k\}$, and colors each $d$-tuple in $\{1, \ldots, k\}^d$ (i.e., $\{1, \ldots, k\} \times \cdots \times \{1,\ldots,k\}$) randomly with a color out of two colors, say 0 and 1, such that the probability of each $d$-tuple being colored with $1$ is $\frac{1}{k}$. Notice the two levels of randomness here and the fact that $k$ is chosen suitably by the algorithm. The main insight is that, when the number of hyperedges is above a threshold, a suitable scaling of 
the number of hyperedges colored with 1, will approximate the number of hyperedges. The case when the number of hyperedges is below a threshold can be taken care of by the exact estimation step. We overcome the bottleneck of arbitrary intersection patterns in case of $d$-uniform hyperedges by the two levels of randomness. 
%}

\subsection{Proof of the lemma}
\begin{proof} We prove this lemma using induction on $d$.
\paragraph*{The base case:} For $d=1$, the hash function is $h_1:[k]\rightarrow \{0,1\}$. The vertices in $A_1$ are \colored with $[k]$. So, $\cR_1=\sum\limits_{c_1 \in [k]}m_o(\chi(1,c_1)) \times h_1(c_1)$. We have $\E[\cR_1]=\frac{m_o(A_1)}{k}$. Note that the set of $1$-uniform hyperedges $\cF_o(A_1)$ is a subset of $A_1$. Let $X_F$ be the indicator random variable, corresponding to each hyperedge $F \in \cF_o(A_1)$, indicating whether the hash function evaluates to $1$  where the only element in $F$ gets color $x \in [k]$. That is, for each hyperedge $F \in \cF_o(A_1)$, $X_F=1$ if and only if $h_1(x)=1$. Therefore, $\pr(X_F=1)=\frac{1}{k}$. Observe that the random variables $X_F$ are mutually independent as $F$ depends only on $A_1$. The number of properly colored hyperedges $\cR_1$ can be expressed as the sum of the mutually independent random variables $X_F$, i.e., $\cR_1=\sum\limits_{F \in \cF_o(A_1)}X_F$. Now, applying Hoeffding's bound (see Lemma~\ref{lem:hoeff_inq} in Appendix~\ref{sec:prelim}), we get 
$$\pr\left(\size{\cR_1-\frac{m_o(A_1)}{k}} \geq  4{\theta} \cdot \sqrt{ \log n \cdot m_o(A_1)}\right) \leq \frac{2}{n^{16\theta^2}}\leq  p_1.$$



\paragraph*{The inductive case:} 
\remove{
Now, consider the following definition of a \emph{properly colored} ordered hyperedge.
\begin{defi} \label{defi:proper-order} An ordered hyperedge $F_o \in \cF_o\left(\chi({1,c_1}),\ldots,\chi({1,c_{a_1}}),\ldots, \chi({s,c_{d-a_s+1}})\ldots \chi({s,c_d})\right)$ is said to be \emph{properly} colored if there exists $(c_1,\ldots,c_d) \in [k]^d$ such that $h_d(c_1,\ldots,c_d)=1$. \end{defi}
}

Observe that the probability that a hyperedge is \emph{properly colored} with a color tuple $(c_1, \ldots, c_d)$ is same as the probability of the hash function evaluating to $1$ for that color tuple and is equal to $\frac{1}{k}$. $\cR_d$, as defined in the statement of Lemma~\ref{lem:sparse2}, represents the number of properly colored hyperedges. So, $\E[\cR_d]=m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})/k$. 

	Note that $A=\cup_{i=1}^sA_i$. Without loss of generality, assume that the vertices in $A$ are $1,\ldots,n'$, where $n'\leq n$. Viewing the coloring process as a random process, let us focus on the instance when, in some arbitrary order, vertices $1,\ldots,t-1$ have been colored and we are exposing the vertex $t$ for coloring, where $2 \leq t \leq n'-1$. Recall that $\cF_o(t)$ denotes the set of ordered hyperedges incident on $t$. We classify the ordered hyperedges $\cF_o(t)$ based on the position of $t$, i.e., let $\cF_o(t,\mu) \subseteq \cF_o(t)$ be the set of ordered hyperedges where $t$ is fixed as the $\mu$-th vertex, $\mu \in [d]$. {As $\size{\cF_o(t)}=d!\cF(t)$ and $\size{\cF_o(t,\mu)}=(d-1)!\cF(t)$}, we have the following observation that will be used later in the proof. 

\begin{obs} \label{obs:mu-edge} $\size{\cF_o(t,\mu)}= \frac{(d-1)! ~ \size{\cF_o(t)}}{d!} = \frac{\size{\cF_o(t)}}{d}$ where $\mu \in [d]$. \end{obs} 

{Next, we bring in a definition that would allow us to capture the randomness in the coloring process when the vertex $t$ is colored.}
\begin{defi}
 An ordered hyperedge $F \in \cF_o(t,\mu)$ is said to be of \emph{type-$\lambda$} if $F$ has exactly $\lambda$ many vertices from the set $[t]$, where $\lambda \in [d]$. 
\label{def:type-lambda}
\end{defi}
To get a sense of the above definition, consider the cases $\lambda < d$ and $\lambda = d$; the second case fixes all vertices in $F$ to be from $[t]$, while in the first case, there is room for vertices beyond $[t]$.
For {$\mu, \lambda \in [d]$}, let $\cF_o^\lambda(t)$ and $\cF_o^\lambda (t,\mu)$ be the set of ordered hyperedges of type-$\lambda$  in $\cF_o(t)$ and $\cF_o(t,\mu)$, respectively. Given that the vertex $t$ is colored with color $c \in [k]$, let $N_c^\lambda(t)$ and $N_c^\lambda(t,\mu)$ be the random variables that denote the number of ordered hyperedges in $\cF_o^\lambda(t)$ and $\cF_o^\lambda(t,\mu)$ that are properly colored, respectively. \remove{
Let $A = [n'] = \{1, \ldots, n'\}$, where $n' \leq n$.} Let $Z_i \in [k]$ be the random variable that denotes the color assigned to the vertex $i \in A~\mbox{(recall $A=\bigcup_{i=1}^s A_i$)} = [n']$, where $n' \leq n$. Note that $\cR_d$ is a function of $Z_1,\ldots,Z_{n'}$, that is, $\cR_d=f(Z_1,\ldots, Z_{n'})$. 

Let $\E_{\cR_d}^t$ denote the difference in the conditional expectation of the number of properly colored ordered hyperedges given that the $t$-th vertex is differently colored by considering the hyperedges in each $\cF_o^\lambda (t,\mu)$, where $\lambda,\mu \in [d]$.

\begin{eqnarray}
	\E_{\cR_d}^t &=& \size{\E \left[ \cR_d~|~Z_1,\ldots,Z_{t-1}, Z_t =\rho \right] - \E \left[ \cR_d~|~Z_1,\ldots,Z_{t-1}, Z_t =\nu \right]} \label{eqn1} \\
	&=& \size{\sum\limits_{\lambda=1}^{d}\E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right] } \label{eqn2}\\
	&=& \size{\left(N_{\rho}^{d}(t) - N_{\nu}^{d}(t)\right)+\sum\limits_{\lambda=1}^{d-1} \E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right] }\\
	&=& \size{\sum\limits_{\mu=1}^d\left(N_{\rho}^{d}(t,\mu) - N_{\nu}^{d}(t,\mu)\right) + \sum\limits_{\lambda=1}^{d-1} \E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right]}\\
	&\leq& \sum\limits_{\mu=1}^d \size{N_{\rho}^{d}(t,\mu) - N_{\nu}^{d}(t,\mu)} + \size{\sum\limits_{\lambda=1}^{d-1} \E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right]}
\end{eqnarray}
Since the hyperedges without having $t$ as one of its vertex have the same contribution to both $\E \left[ \cR_d~|~Z_1,\ldots,Z_{t-1}, Z_t =\rho \right]$ and $\E \left[ \cR_d~|~Z_1,\ldots,Z_{t-1}, Z_t =\nu \right]$, Equation~\ref{eqn2} follows from Equation~\ref{eqn1}. 

Now, consider the following claim. 
\begin{cl} \label{cl:inter_sparse}
	\begin{itemize}
		\item[(a)] $\pr\left(\size{ N_{\rho}^{d}(t,\mu) - N_{\nu}^{d}(t,\mu)} \leq 2^{2d-1}\theta^{d-1} \sqrt{{(d-1)!\cF_o(t,\mu)}\log^{d-1} n}\right) \geq 1-2p_{d-1}$, where $\mu \in [d]$ and $\theta > d$ is the constant mentioned in the statement of Lemma~\ref{lem:sparse2}. 
		\item[(b)] $\E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right]=0,~\forall\lambda \in [d-1]$.
	\end{itemize}
\end{cl}

\begin{proof}[Proof of Claim~\ref{cl:inter_sparse}]
\begin{itemize}
	\item[(a)] For simplicity, we argue for $\mu =1$, i.e., $t$ appears at the first position. However, the argument will be similar for any $\mu\in [d]$. Consider a $(d-1)$-uniform hypergraph $\cH'$ such that $U(\cH')=\{1,\ldots,t-1\}$%\complain{(Gopi, does this notation $U(\cH')=[t-1]$ make sense?)} 
 and $\cF_o(\cH')=\{(x_1,\ldots,x_{d-1}):(t,x_1,\ldots,x_{d-1})\in \cF_o^d(t,1)\}$. Let $h_{d-1}:[k]^{d-1} \rightarrow \{0,1\}$ be a hash function such that $h_{d-1}(x_1,\ldots,x_{d-1})=h_d(t,x_1,\ldots,x_d)$. Observe that $\pr(h_{d-1}({\bf a})=1) =\frac{1}{k}$ for each tuple ${\bf a} \in [k]^{d-1}$. Consider the $(d-1)$-partite hypergraph $\cH'\left(B_1^{[a_1-1]}B_2^{[a_2]}\cdots B_s^{[a_s]}\right)$, where $B_i = A_i \cap [t-1]$~\footnote{Recall that $B^{[b]}$ denotes $B...B$($b$ times).}. Observe that $m_o\left(B_1^{[a_1-1]}B_2^{[a_2]}\cdots B_s^{[a_s]}\right)=\size{\cF_o^d(t,1)}$. Recall that the vertices in $\cup_{i=1}^s A_i$ are \colored with $[k]$. Let $\chi'(i,j)=\{v \in B_i:\mbox{$v$ is \colored with color $j$}\}$. Let
		$$\cR_{d-1}=\sum\limits_{(c_1,\ldots,c_{d-1}) \in [k]^{d-1}} m_o\left(\chi'({1,c_1}),\ldots,\chi'({1,c_{a_1-1}}),\ldots, \chi'({s,c_{d-a_s}})\ldots \chi'({s,c_{d-1}})\right)\times h_{d-1}(c_1,\ldots,c_{d-1})$$
%\complain{Gopi, check the indices of the color classes once more to see if they are ok?}
Observe that the random variables $N_\rho^d(t,1)$ and $N_\nu^d(t,1)$ follow the distribution of the random variable $\cR_{d-1}$. By the induction hypothesis, 
$$\pr\left(\size{\cR_{d-1}-\frac{m_o\left(B_1^{[a_1-1]}B_2^{[a_2]}\cdots B_s^{[a_s]}\right)}{k}} \geq  2^{2d-2}\theta^{d-1} \sqrt{{(d-1)! m_o\left(B_1^{[a_1-1]}B_2^{[a_2]}\cdots B_s^{[a_s]}\right)}\log^{d-1} n}\right) \leq p_{d-1}$$

Using $m_o\left(B_1^{[a_1-1]}B_2^{[a_2]}\cdots B_s^{[a_s]}\right)=\size{\cF_o^d(t,1)}$, we have
 \begin{equation}
  \label{eqn:ind}
	 \pr\left(\size{\cR_{d-1} - \frac{\size{\cF_o^d(t,1)}}{k}} \geq  2^{2d-2}\theta^{d-1} \sqrt{{(d-1)!\cF^d_o(t,1)}\log^{d-1} n}\right) \leq p_{d-1}
 \end{equation}

Using the above equation, the claim follows using the following. 

		$$\pr\left(\size{ N_{\rho}^{d}(t,1) - N_{\nu}^{d}(t,1)} \geq 2^{2d-1}\theta^{d-1} \sqrt{{(d-1)!\cF_o(t,1)}\log^{d-1} n}\right) \leq 2 p_{d-1}.$$ 
		
Let $L=2^{2d-1}\theta^{d-1} \sqrt{{(d-1)!\cF_o(t,1)}\log^{d-1} n}$. Now, 
\begin{eqnarray*}
	&&\pr\left(\size{ N_{\rho}^{d}(t,1) - N_{\nu}^{d}(t,1)} \geq 2^{2d-1}\theta^{d-1} \sqrt{{(d-1)!\cF_o(t,1)}\log^{d-1} n}\right) \\
	&\leq& \pr\left(\size{N_{\rho}^{d}(t,1) -\frac{\size{\cF_o^d(t,1)}}{k}} \geq \frac{L}{2} \right) + \pr\left(\size{N_{\nu}^{d}(t,1) -\frac{\size{\cF_o^d(t,1)}}{k}} \geq \frac{L}{2} \right)\\
	&=& 2 \cdot \pr\left(\size{N_{\rho}^{d}(t,1) -\frac{\size{\cF_o^d(t,1)}}{k}} \geq  2^{2d-2}\theta^{d-1} \sqrt{{(d-1)!\cF_o(t,1)}\log^{d-1} n}\right) \\
	&\leq& 2\cdot \pr\left(\size{N_{\rho}^{d}(t,1) -\frac{\size{\cF_o^d(t,1)}}{k}} \geq 2^{2d-2}\theta^{d-1} \sqrt{{(d-1)!\cF^d_o(t,1)}\log^{d-1} n}\right)~~~~(\because \cF_o^d(t,1) \leq \cF_o(t,1))\\
	&\leq& 2p_{d-1}~~~~(\mbox{By Equation~\ref{eqn:ind}})
\end{eqnarray*}


\item[(b)]First, consider the case when $t$ is \colored with color $\rho$. For $F \in \cF_o^\lambda(t), \lambda \in [d-1]$, let $X_F$ be the indicator random variable such that $X_F=1$ if and only if $F$ is properly colored. As $F$ is of type $\lambda$, there exists at least one vertex in $F$ that is not colored yet, that is, $\pr(X_F=1)=\frac{1}{k}$. Observe that $N^\lambda_\rho(t)=\sum\limits_{F \in \cF_o^\lambda(t)}X_F$. Hence, $\E\left[N^\lambda_\rho(t)\right]=\size{\cF_o^\lambda(t)}/k$. Similarly, one can show that $\E\left[N^\lambda_\nu(t)\right]=\size{\cF_o^\lambda(t)}/k$. Hence, $\E\left[ N_{\rho}^{\lambda}(t) - N_{\nu}^{\lambda}(t) \right]=0$.
\end{itemize}

\end{proof}




Now, let us come back to the proof of Lemma~\ref{lem:sparse2}. By Claim~\ref{cl:inter_sparse} and Observation~\ref{obs:mu-edge}, we have the following with probability at least $1-2d\cdot p_{d-1}$.
\begin{eqnarray*}
\E^t_{\cR_d} &\leq& 2^{2d-1}\theta^{d-1} \cdot d \cdot \sqrt{(d-1)!\frac{\cF_o(t)}{d} \log^{d-1} n} =  2^{2d-1}\theta^{d-1} \sqrt{{d!\cF_o(t)} \log^{d-1} n}=c_t,
\end{eqnarray*}
where $c_t= 2^{2d-1}{\theta}^{d-1} \sqrt{{d!\cF_o(t)} \log^{d-1} n}$. 

Let $\cB$ be the event that there exists $t \in [n]$ such that $\E_{\cR^d}^t > c_t$. By the union bound over all $t \in [n]$, $\pr(\cB) \leq 2dnp_{d-1}={2dn}\frac{{(d-1)!}}{n^{4\theta-2(d-1)}}\leq \frac{2d!}{n^{4\theta-2d+1}}$. Using the method of \emph{averaged bounded difference}~\cite{DubhashiP09} (See Lemma~\ref{lem:dp} in Appendix~\ref{sec:prelim}), we have 
$$ \pr\left(\size{\cR_d - \E[\cR_d]} >\delta + m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})\pr(\cB) \right) \leq e^{-{\delta^2}/{\sum\limits_{t=1}^{n} c_t^2}} + \pr(\cB)$$

We set $\delta = 2 \sqrt{\theta \log n \cdot \sum\limits_{t \in [n]}c_t^2}=2^{2d}\theta^{d-1/2}  \sqrt{d!m_o(\ssubset)\log ^d n}$. Using $m_o(\ssubset) \leq n^d$ and $\pr(\cB) \leq \frac{2d!}{n^{4\theta -4d+1}}$ , we have 
\begin{eqnarray*}
	&& \pr\left(\size{\cR_d-\frac{m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})}{k}} > 2^{2d} \theta^{d-1/2} \sqrt{d! m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]}) \log ^d n}+\frac{2d!n^d}{n^{4\theta -2d+1}}\right) \\
	&\leq& \frac{1}{n^{4\theta}}+\frac{2d!}{n^{4\theta-2d+1}}
\end{eqnarray*}
Assuming $n \gg d$, 
$ \pr\left(\size{\cR_d - \frac{m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]})}{k}} \geq 2^{2d} \theta ^d\sqrt{d! m_o(A_1^{[a_1]},\ldots,A_s^{[a_s]}) \log ^d n}  \right) \leq \frac{d!}{n^{4\theta -2d}}=p_{d} $
\end{proof}


==> tech-overview.tex <==
\section{Technical Overview} \label{sec:overview}
\noindent
We briefly describe the overview of our work and put our work in context with recent works. 
\subsection{The context of our work}
\noindent Beame \etal~\cite{BeameHRRS18} developed a framework to estimate the number of edges in a graph using \bis queries. This framework involves subroutines for sparsifying a graph into a number of subgraphs each with reduced number of edges, and exactly or approximately counting the number of edges in these subgraphs. Sparsification constitutes the main building block of this framework. The sparsification routine of Beame \etal~randomly colors the vertices of a graph with $2k$ colors. Let $A_i$ denote the set of vertices colored with color $i$. Beame \etal~argued that the sum of the number of edges between $A_i$ and $A_{k+i}$ for $1\leq i\leq k$ approximates the total number of edges in the graph within a constant factor with high probability. Therefore, the original problem reduces to the problem of counting the number of edges in bipartite subgraphs. Here, we have $k$ bipartite subgraphs and it suffices to count the number of edges in these bipartite subgraphs. With this method, they obtained a query complexity of $O(\eps^{-4} \log^{14} n)$ with high probability.

Bhattacharya \etal~\cite{BhattaISAAC} extended this framework to estimate the number of triangles in a graph using \tis queries, where given three disjoint subsets of vertices $A, \, B, \, C$, a \tis query with inputs $A, \, B, \, C$ answers whether there exists a triangle with one endpoint in each of $A,B,C$. The sparsification routine now requires to color the vertices randomly using $3k$ colors and counts the number of properly colored triangles where a properly colored triangle has one endpoint each in $A_i$, $A_{k+i}$, and $A_{2k+i}$ for any $1\leq i\leq k$. Unlike the scenario in Beame \etal~where two edges intersect in at most one vertex, here two triangles can share an edge. Therefore, the random variables used to estimate the number of {\it properly colored} triangles are not independent. Bhattacharya \etal~estimated the number of triangles assuming that the number of triangles incident on any edge is bounded by a parameter $\Delta$. In this way, they obtained a query complexity of $O(\eps^{-12} \Delta^{12} \log^{25}n)$.

In this paper, we fully generalize the frameworks of Stockmeyer~\cite{Stockmeyer83,Stockmeyer85}, Ron and Tsur~\cite{RonT16}, Beame \etal~\cite{BeameHRRS18} and Bhattacharya~\etal~\cite{BhattaISAAC} to estimate the number of hyperedges in a $d$-uniform hypergraph using \gpis queries. \remove{We do not have the dependency problem for estimating the number of hyperedges in a hypergraph because existence of one hyperedge does not imply anything about the existence of another hyperedge with a subset of its vertices.}

